One-Shot Domain Adaptation For Face Generation

In this paper, we propose a framework capable of generating face images that fall into the same distribution as that of a given one-shot example. We leverage a pre-trained StyleGAN model that already learned the generic face distribution. Given the one-shot target, we develop an iterative optimization scheme that rapidly adapts the weights of the model to shift the output's high-level distribution to the target's. To generate images of the same distribution, we introduce a style-mixing technique that transfers the low-level statistics from the target to faces randomly generated with the model. With that, we are able to generate an unlimited number of faces that inherit from the distribution of both generic human faces and the one-shot example. The newly generated faces can serve as augmented training data for other downstream tasks. Such setting is appealing as it requires labeling very few, or even one example, in the target domain, which is often the case of real-world face manipulations that result from a variety of unknown and unique distributions, each with extremely low prevalence. We show the effectiveness of our one-shot approach for detecting face manipulations and compare it with other few-shot domain adaptation methods qualitatively and quantitatively.

==> backup.tex <==
\begin{figure}[!h]
\centering
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cccc}
  \multicolumn{2}{c}{$I_1$\includegraphics[width=.12\textwidth]{figures/combine/ashish_01.png}} & \multicolumn{2}{c}{$I_2$\includegraphics[width=.12\textwidth]{figures/combine/alex_01.png}} \\
  i=1\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_1_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_1_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_1_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_1_into_ashish_at_-1.jpg} \\ 
  i=2\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_2_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_2_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_2_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_2_into_ashish_at_-1.jpg} \\ 
  i=3\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_3_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_3_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_3_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_3_into_ashish_at_-1.jpg} \\ 
  i=4\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_4_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_4_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_4_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_4_into_ashish_at_-1.jpg} \\ 
  i=5\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_5_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_5_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_5_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_5_into_ashish_at_-1.jpg} \\ 
  i=6\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_6_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_6_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_6_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_6_into_ashish_at_-1.jpg} \\ 
  i=7\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_7_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_7_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_7_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_7_into_ashish_at_-1.jpg} \\ 
  i=8\includegraphics[width=.12\textwidth]{figures/combine/insert_alex_8_into_ashish_at_1.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_8_into_ashish_at_3.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_8_into_ashish_at_4.jpg} &
  \includegraphics[width=.12\textwidth]{figures/combine/insert_alex_8_into_ashish_at_-1.jpg} \\ 
   j=1 & j=2& j=4 & j=-1\\
\end{tabular}
\caption{Top row: two images $I_1$ and $I_2$ as input. Bottom rows: replace $i$ layers starting from $j_{th}$ layer of $s_1$ (inferred from $I_1$) with those of $s_2$ (inferred from $I_2$) and regenerate the image. j=-1 (last column) means replacing the $i$ layers at the end.}
\label{fig:combine}
\end{figure}

==> intro_bak.tex <==
\section{Introduction}
Deep learning has been prevailing in a variety of computer vision tasks, especially in supervised settings such as learning for classification, detection or segmentation~\cite{he2016deep,ren2015faster,liu2016ssd,he2017mask}. Deep generative models such as Variational AutoEncoder (VAE)~\cite{kingma2013auto,lombardi2018deep} and Generative Adversarial Networks (GAN)~\cite{goodfellow2014generative,olszewski2017realistic,thies2016face2face,faceswap,df_github,zollhofer2018state} in particular have gained significant prominence in the field of deep learning due to their ability to generate highly realistic images depicting faces, natural scenes and objects.

Recent advances in deep learning have paved the way for many important applications ranging from super resolution, movie making, game development, cross domain style transfer, face synthesis and aging prediction, image inpainting, photo editing and others. However, the advent of DL has also precipitated the emerging of applications that abuse its power. Technologies such as Face2Face~\cite{thies2016face2face}, FaceSwap~\cite{faceswap}, and encoder-decoder DeepFake~\cite{df_github} have resulted in the emergence of online impersonations/fabrication of news, threatening even to sway the outcomes of elections.


\begin{figure}[!t]
\centering
\small
\setlength{\tabcolsep}{1pt}
\begin{tabular}{cc}
  \includegraphics[width=.24\textwidth]{figures/qual_results_new/ae/ori_stylegan.jpg} &
  \includegraphics[width=.24\textwidth]{figures/qual_results_new/ae/autoencoder.png} \\
  (a) & (b) \\
  \includegraphics[width=.24\textwidth]{figures/qual_results_new/ae/synthesized.jpg} &
  \includegraphics[width=.24\textwidth]{figures/qual_results_new/ae/reconstructed.png} \\
  (c) & (d) \\
\end{tabular}
\caption{One-shot domain adaptation on encoder-decoder DeepFake using StyleGAN generator. (a). A Random StyleGAN generated image. (b). A one-shot image from encoder-decoder DeepFake of DFDC~\cite{dolhansky2019deepfake}. (c). A StyleGAN generated image using the same random latent input as (a) after domain adaptation. (d). The StyleGAN reconsutrcted one-shot DeepFake after domain adaptation.}
  \vspace{-5pt}
\label{fig:teaser}
\end{figure}


In this paper, we are interested in detecting Deepfakes, which refers to manipulations to replace the human face of authentic media by the face of a different person~\cite{rossler2019faceforensics++,chesney2018deep,dolhansky2019deepfake}. This is often coupled with malicious intent of defaming other people or spreading fabricated news. Image generations have been trending as a popular research topic due to the rising prevalence and public interest in Deepfake. As a result, many techniques for generating images have been proposed, each with specific probabilistic distributions or fingerprints. Often times, a new type of synthetic images emerges online but the underlying techniques are unknown, and only a few bespoke examples exist. Training a classifier to detect them poses significant challenges as we are unable to infer the complete probabilistic distribution.

To this end, our method aims to mimic a complete distribution of the target domain given just one example. While most existing domain adaptation approaches try to find a feature space in which there is maximum confusion between source and target distributions~\cite{liu2018unified,motiian2017unified}, we directly manipulate the distribution in the image space. We first train a deep generative model to learn the generic probabilistic distribution of human faces on a large collection of face images. Specifically, we adopt Style-based Generator (StyleGAN)~\cite{karras2019style} given its high capacity and superior generation quality. With the trained StyleGAN model and a single example from a specific distribution, we run iterative optimization of the input style vector to project the image to the StyleGAN distribution, followed by optimizing the model weights to minimize the projection distance and shift the StyleGAN distribution to the target's. We are then able to generate an unlimited number of random faces that are from a similar distribution as the target and yet preserve the manifold of the generic human face distributions. We further transfer low-level style from the one-shot target to the StyleGAN generated images. To do so, we notice the style vector of a given image has hierarchical structures and represents different attributes at different style layers. If we replace the style vector of randomly synthesized images with the style vector of the target at late layers, we are able to transfer the low-level statistics from the target domain to the random images we generated. We refer to this procedure as style-mixing. Combining iterative weight optimization with style-mixing, the generated images not only capture the overall probabilistic distribution of the target domain but also resemble the one-shot image in low-level appearances and details. Finally, one can then use the generated images to train a model for detecting images from the target domain.  Extensive experiment shows that our detector achieves significantly improved accuracy compared with the baseline and other state-of-the-art few-shot domain adaptation and image translation techniques. 

Our contributions can be summarized as follows:
\begin{enumerate}
	\item We introduce a novel one-shot domain adaptation framework that is effective at training a face manipulation detector given a single example of a specific face manipulation distribution. 
	\item We demonstrate that the images generated with our approach, when utilized to train a classifier, achieves superior performance in telling apart real and manipulated face images.
\end{enumerate}

